Feedback between microscopic activity and macroscopic dynamics drives excitability and oscillations in mechanochemical matter

The macroscopic behaviour of active matter arises from nonequilibrium microscopic processes. In soft materials, active stresses typically drive macroscopic shape changes, which in turn alter the geometry constraining the microscopic dynamics, leading to complex feedback effects. Although such mechanochemical coupling is common in living matter and associated with biological functions such as cell migration, division, and differentiation, the underlying principles are not well understood due to a lack of minimal models that bridge the scales from the microscopic biochemical processes to the macroscopic shape dynamics. To address this gap, we derive tractable coarse-grained equations from microscopic dynamics for a class of mechanochemical systems, in which biochemical signal processing is coupled to shape dynamics. Specifically, we consider molecular interactions at the surface of biological cells that commonly drive cell-cell signaling and adhesion, and obtain a macroscopic description of cells as signal-processing droplets that adaptively change their interfacial tensions. We find a rich phenomenology, including multistability, symmetry-breaking, excitability, and self-sustained shape oscillations, with the underlying critical points revealing universal characteristics of such systems. Our tractable framework provides a paradigm for how soft active materials respond to shape-dependent signals, and suggests novel modes of self-organisation at the collective scale. These are explored further in our companion paper [arxiv 2402.08664v3].

==> sm.tex <==
\appendix
\section{Statistical physics of adhesion molecule binding}
\label{sec:adhesion_statmech}

At steady-state, the flux coupling bulk and surface concentrations [Eq.~\eqref{eq:bc_flux}] vanishes and the surface can be considered to be in chemical and thermal equilibrium with a constant temperature $T$ and in contact with a bath of constant chemical potential $\mu=\mu(c_\mathrm{N})$ set by the steady-state bulk concentration. Note that the chemical potential is kept constant through a non-equilibrium process~--~the turnover of adhesion molecules. Each binding site at the interface is a two-state system: a binding site is either occupied or unoccupied. If $n$ is the number of occupied binding sites, $n^\mathrm{max}$ the total number of available binding sites at the surface and $\epsilon$ the binding energy, then the grand canonical partition sum for the whole surface reads
\begin{align}
    \Xi = \sum_{n=0}^{n^\mathrm{max}} \binom{n^\mathrm{max}}{n}e^{\beta n(\mu-\epsilon)} = \left( 1+e^{\beta(\mu-\epsilon)} \right)^{n^\mathrm{max}}
\end{align}
with $\beta=(k_{\mathrm{B}} T)^{-1}$. The ensemble average of the number of occupied binding sites is
\begin{align}
    \langle n \rangle = \frac{1}{\beta} \frac{\partial \ln \Xi}{\partial\mu} = \frac{n^\mathrm{max}}{1+e^{\beta(\epsilon - \mu)}},
    \label{eq:fermi_dirac}
\end{align}
showing that the system follows Fermi-Dirac statistics. In the chemical equilibrium, the rates of binding and unbinding must be equal for each binding site. The binding rate of adhesion molecules is
\begin{align}
    k_\mathrm{binding} = k_\mathrm{on}^\mathrm{N} c_\mathrm{N} p_\mathrm{uoc}
    \label{eq:k_binding}
\end{align}
with $p_\mathrm{uoc}=1/(1+e^{\beta(\mu - \epsilon)})$ the probability that a binding site is not occupied, while the unbinding rate is
\begin{align}
    k_\mathrm{unbinding} = k_\mathrm{off}^\mathrm{N} p_\mathrm{oc}
    \label{eq:k_unbinding}
\end{align}
with $p_\mathrm{oc} = e^{\beta(\mu - \epsilon)}/(1+e^{\beta(\mu - \epsilon)})$ the probability that a binding site is occupied. From $k_\mathrm{binding} = k_\mathrm{unbinding}$ and Eqs.~\eqref{eq:k_binding}--\eqref{eq:k_unbinding} follows
\begin{align}
    \frac{k_{\mathrm{off}}^{\mathrm{N}}}{k_{\mathrm{on}}^{\mathrm{N}} c_{\mathrm{N}}} = e^{\beta(\epsilon - \mu)}.
\end{align}
From $m_\mathrm{N} = \langle n \rangle/A_\mathrm{c}$ and $m_\mathrm{N}^\mathrm{max} = n^\mathrm{max}/A_\mathrm{c}$ together with Eq.~\eqref{eq:fermi_dirac} and $c_{\rm{N}}=k_{\rm{p}}^{\rm{N}}/k_{\rm{d}}^{\rm{N}}$ follows then Eq.~\eqref{eq:mN}.

\section{Symmetry-breaking of signaling states}
\label{sec:approximation_PF}
In many biological systems, Notch signals are mutually inhibitory, i.e. signals suppress the production of ligands \cite{sjoqvist2019say}. Strong mutual inhibitory interactions generically lead to spontaneous symmetry-breaking \cite{pisarchik2022multistability}, whereby small initial differences in the signaling states are amplified and diverge to high- and low-value steady states. At the onset of symmetry-breaking, the uniform steady-state solution of Eq.~\ref{eq:u_ode} becomes unstable. To derive an approximation for the onset of symmetry-breaking, we expand $\sigma(s_{i})$ [Eq.~\eqref{eq:sigma}] for a general Hill coefficient $h$ to first order around the inflection point $s_{i}=1$ 
\begin{align}
    \sigma(s_{i}) = \frac{1}{2} + \frac{h}{4}(s_{i} - 1) + \mathcal{O}((s_{i}-1)^2)
\end{align}
yielding the dynamic equation
\begin{align}
    \tau_{\rm{u}} \frac{du_i}{dt} = \frac{1}{2} + \frac{h}{4}(s_{i} - 1) - u_i
    \label{eq:u_ode_aprrox}
\end{align}
and using the definition of the signal Eq.~\eqref{eq:signal_definition_doublet} the uniform steady-state is [Fig.~\ref{fig:symmetry_breaking}(a)]
\begin{align}
    u^* = 1 - \frac{2+h}{4 + h \chi \dfrac{A_{\rm{c}}}{A_0}}.
    \label{eq:uniform_steady_states}
\end{align}
Linear stability analysis reveals that this uniform steady state looses stability for
\begin{align}
    \chi_{\mathrm{PF}} = \frac{4 A_0}{h A_{\mathrm{c}}},
    \label{eq:symmetry_breaking_scaling}
\end{align}
with $A_{\mathrm{c}}=A_{\mathrm{c}}(\gamma_{\mathrm{c}})$ and $\gamma_{\mathrm{c}} = \gamma_0 - \gamma_{\mathrm{A}}(u^*)^2$. 
Comparison with the steady-state contact area computed numerically along the supercritical pitchfork bifurcation line that was derived via continuation in MatCont shows good agreement [Fig.~\ref{fig:symmetry_breaking}(b)]. Figure~\ref{fig:SteadyStateContactArea} shows the normalized steady-state contact area $A_{\rm{c}}/A_0$ in the state space of feedback parameters.

\section{Shapes of asymmetric droplets}
\label{sec:shape_asymmetric_droplets}

\begin{figure*}
    \centering
    \includegraphics{Figures/asymmetric_doublet_parameterization.png}
    \caption{ (a) Parameterization of a pair of asymmetric droplets adapted from \cite{maitre2016asymmetric}. (b) The droplet volumes can be expressed in terms of the three spherical cap volumes  $v_1,v_2,v_{\rm{c}}$ (c) Differences in droplet volumes $\delta V/\bar{V}=\{0.25,0.5\}$ (blue) or outer interfacial tensions $\delta \gamma_{\rm{f}}/\bar{\gamma_{\rm{f}}}=\{0.25,0.5\}$ (brown) change how the contact area between the droplets depends on the tension ratio $\gamma_{\rm{c}}/2\bar{\gamma}_{\rm{f}}$. Curves are obtained by numerically minimizing Eq.~\eqref{eq:energy_asymmetric_doublet_2} (Sec.~\ref{sec:numerical_methods} for details) }
    \label{fig:asymmetry_doublet_parameterization}
\end{figure*}

For pairs of droplets with unequal volumes ($V_1 \neq V_2$) or outer surface tensions ($\gamma_{\rm{f},1} \neq \gamma_{\rm{f},2}$), Eq.~\eqref{eq:contact_area} does not describe the size of the contact area. To derive the equilibrium shape and contact size of asymmetric droplets, we compute the minimum of the surface energy
\begin{align}
    E = \gamma_{\rm{c}} A_{\rm{c}} + \gamma_{\rm{f},1} A_{\rm{f},1} +  \gamma_{\rm{f},2} A_{\rm{f},2}
    \label{eq:energy_asymmetric_doublet}
\end{align}
under constant volume constraint. We follow the approach and use the parameterization introduced in \cite{maitre2016asymmetric}, which is shown in Fig.~\ref{fig:asymmetry_doublet_parameterization}(a). The droplet volumes can be expressed in terms of three spherical cap volumes $v_i$ with $i\in\{1,2,\rm{c}\}$ [Fig.~\ref{fig:asymmetry_doublet_parameterization}(b)] such that
\begin{align}
    V_1 = v_1 + v_c \\
    V_2 = v_2 - v_c.
\end{align}
Given the radii of curvature $R_i$ and the radius $r$ as shown in Fig.~\ref{fig:asymmetry_doublet_parameterization}(a), we can define the length scales
\begin{align}
    a_i = \sqrt{R_i^2 - r^2}
\end{align}
and surfaces
\begin{align}
    H_i(a_i, r) = \frac{1}{2}\left( a_i^2 + r^2 + a_i \sqrt{a_i^2 + r^2} \right),
\end{align}
which allows to express the spherical cap volumes as
\begin{align}
    v_i(a_i, r) = \frac{\pi}{3} \left(a_i + \sqrt{a_i^2 + r^2}\right)^2 \left(2 \sqrt{a_i^2 + r^2} - a_i \right)
\end{align}
and the different droplet surfaces as 
\begin{align}
    A_i(a_i, r) = 4 \pi H_i(a_i, r).
\end{align}
Using these definitions and expressing the outer surface tensions as $\gamma_{\rm{f},1} = \bar{\gamma}_{\rm{f}} + \delta \gamma_{\rm{f}}, \gamma_{\rm{f},2} = \bar{\gamma}_{\rm{f}} - \delta \gamma_{\rm{f}}$, we can rewrite Eq.~\eqref{eq:energy_asymmetric_doublet} as
\begin{align}
    \frac{E}{4 \pi \bar{\gamma}_{\rm{f}}} &= 
    \left(1 + \frac{\delta \gamma_{\rm{f}}}{\bar{\gamma}_{\rm{f}}} \right) H_1(a_1,r)
    +  \left(1 - \frac{\delta \gamma_{\rm{f}}}{\bar{\gamma}_{\rm{f}}} \right) H_2(a_2,r) \nonumber \\
     &+  2 \left(\frac{ \gamma_{\rm{c}} }{2 \bar{\gamma}_{\rm{f}}} \right) H_{\rm{c}}(a_{\rm{c}},r)
     \label{eq:energy_asymmetric_doublet_2}
\end{align}
with $\bar{\gamma}_{\rm{f}} = (\gamma_{\rm{f},1} + \gamma_{\rm{f},2})/2$. The minima in terms of the four parameters ($a_1,a_2,a_{\rm{c}},r$) under constant volume constraints $V_1 = \bar{V} - \delta V, V_2 = \bar{V} + \delta V$ were computed numerically, allowing to derive the size of the contact area $A_{\rm{c}}=4\pi H_c(a_c,r)$ (Sec.~\ref{sec:numerical_methods}).

\section{Numerical methods}

\begin{table*}[ht!]
    \centering
    \begin{tabular}{|p{70 mm}|p{20 mm}|p{60mm}|}
        \hline
         Physical quantity & Symbol & Values\\
         \hline
         Base line interfacial tension relative to outer surface tension in a single adherent droplet & $(\gamma_0-\gamma_{\rm{m}})/2\gamma_{\rm{f}}$ & Fig.~\ref{fig:3}(a,c): 0.95 \hfill\newline \\
         \hline
         Base line interfacial tension relative to outer surface tension & $\gamma_0/2\gamma_{\rm{f}}$ & 
         Fig.~\ref{fig:4}(a): 0.9 \hfill\newline 
         Fig.~\ref{fig:4}(c): 0.7 \hfill\newline
          Fig.~\ref{fig:5}-\ref{fig:7},\ref{fig:symmetry_breaking},\ref{fig:SteadyStateContactArea}: 0.98 \hfill\newline
         \\
         \hline Reference susceptibility & $\chi_0$ & 
         Fig.~\ref{fig:3}: $\chi_0^{\rm{cusp}} = 2.8612$ \hfill \newline
         Fig.~\ref{fig:4}: $\chi_0^{\rm{PF}} = 16.629$ \hfill \newline
         Fig.~\ref{fig:5}-\ref{fig:7},\ref{fig:SteadyStateContactArea}: $\chi_0 = 40.604$
         \hfill \newline
         \\
         \hline
         Adaptive adhesion coefficient relative to outer surface tension & $\gamma_{\rm{A}}/2\gamma_{\rm{f}}$ & 
         Fig.~\ref{fig:3}(a, inlet): 0.9 \hfill \newline
         Fig.~\ref{fig:4}(a, inlet): 0.8 \hfill \newline
         Fig.~\ref{fig:5}(b): \{square, triangle: 0.15, quarterfoil:0.21, star:0.23, plus:0.2352, pentagon:0.5\} \hfill \newline
         
         Fig.~\ref{fig:5}(d): 0.8 \hfill \newline 
          Fig.~\ref{fig:5}(e,f): \{0.4, 0.6, 0.8\} 
          Fig.~\ref{fig:7}(b): 0.637 \hfill \newline
          Fig.~\ref{fig:7}(c): \{0.245, 0.637\} \hfill \newline\\%\hfill\newline
         % Fig.~\ref{fig:asymmetric_doublets_results}(c): 0.65 \\
         \hline
         Relative signal susceptibility & $\chi/\chi_0$ &
         Fig.~\ref{fig:4}(a, inset): 2.8 \hfill \newline
         Fig.~\ref{fig:5}(b): \{square:0.1, quarterfoil:0.61, star:0.604, cross:0.6021, pentagon:0.6, triangle:0.95\} \hfill \newline
         Fig.~\ref{fig:5}(c): \{0.62,0.665,0.68\} \hfill \newline
         Fig.~\ref{fig:5}(d): \{0.4704, 0.7388\} \hfill \newline
         Fig.~\ref{fig:7}(c): \{0.3,0.465,0.4885 0.5,0.5221 0.6, 0.74,0.9 \}
         \\
         \hline
        Volume asymmetry & $\delta V/\bar{V}$ & Fig.~\ref{fig:6}: \{0.25, 0.5\} \\
         \hline
         Tension asymmetry & $\delta \gamma_{\rm{f}}/ \bar{\gamma}_{\rm{f}}$ & Fig.~\ref{fig:6}: \{0.25, 0.5\} \\
         \hline
         Hill coefficient & $h$ & 
         Fig.~\ref{fig:3}(a,b): 2 \hfill \newline
         Fig.~\ref{fig:4}(a-c): 2 \hfill \newline
         Fig.~\ref{fig:5}-\ref{fig:7}: 4 \hfill \newline
         \\
         \hline
    \end{tabular}
    \caption{Parameter values.}
    \label{tab:parameter_values_figures}
\end{table*}

\label{sec:numerical_methods}

\subsection{Bifurcation analysis}
The state and bifurcation diagrams presented in Fig.~\ref{fig:5}(a),(c),%Fig.~\ref{fig:asymmetric_doublets_results}(a),(b)
%and Fig.~\ref{fig:SPDetails} 
were computed via continuation with the MATLAB-based software package MatCont \cite{dhooge2008new} (MatCont7p3 and MATLAB R2021a, scripts with details and numerical settings available at \textcolor{red}{link}). In general, initial fixpoints to initialize the continuation were computed by integration over time with random initial conditions using the Integrator Method ode45. 

%The saddle-node homoclinic (HSN) and associated non-central homoclinic to saddle-node (NCH) bifurcations [Fig.3~\ref{fig:asymmetric_doublets_results}(b)] could only be obtained using the GUI-based version of MatCont7p3. For this, continuation of limit cycles was performed for $\gamma_{A}/\gamma_0=0.95$ and decreasing continuation parameter $\chi$ until the period reached a value close to 100 indicating the presence of a homoclinic causing period divergence. For different values of $\gamma_{A}/\gamma_0=0.95$, this point consistently coincides with the saddle-node bifurcation line. From the limit cycle of largest period, continuation of a HSN was initialized with InitStepsize 0.01, MinStepsize 0.05, MaxStepsize 0.1, MaxNewtonIters 3, MaxCorrIters 10, MaxTestIters 10, VarTolerance 1e-6, FunTolerance 1e-6, TestTolerance 1e-5, Adapt 1, MaxNumPoints 2000, CheckClosed 50 and Jacobian Increment 1e-05. Continuation of the HSN allows to detect the NCH codimension 2 point.\\

Results of the continuation were confirmed using simulations and analysis in Mathematica 13.0 (notebook available at \textcolor{red}{link}). Specifically, we tested the number and types of stable attractors in different parameter regimes with simulations using NDSolve and ParametricNDSolve with the equation simplification method \emph{Residuals}. Fixpoints shown in the phase plots Fig.~\ref{fig:5}(b) were computed numerically in Mathematica from the intersections of nullclines. The SHET [Fig.~\ref{fig:5}(b)], HSN and Hom [Fig.~\ref{fig:7}(b)] were computed from simulation trajectories at parameter values very close to the bifurcation point. The oscillation amplitude [Fig.~\ref{fig:5}(d),(e)] and period  [Fig.~\ref{fig:5}(a)] were computed from the extrema of simulated trajectories, and checked against the dominant Fourier components.\\

\subsection{Timescale of symmetry-breaking}

The time of symmetry-breaking  $T_{\rm{sym}}$ [Fig.~\ref{fig:2}(b),blue curve] was computed as the simulation time (Mathematica) until 99\% of the steady-state internal state difference $|u_1-u_2|$ is reached, starting from initial conditions $(u_1,u_2)=(0.01,0.02)$. The saddle  and its eigenvalues [Fig.~\ref{fig:2}(b),red crosses] were found numerically in Mathematica from the intersections of nullclines. Eigenvalues were normalized against the maximum saddle eigenvalue at $\chi/\chi_0^{\rm{PF}}=2, \gamma_{\rm{A}}/\gamma_0 = 1$.

\subsection{Treatment of asymmetric droplet shapes}
To obtain estimates of the equilibrium shapes of asymmetric droplets, we numerically computed the minimum of Eq.~\eqref{eq:energy_asymmetric_doublet_2} in terms of the four parameters ($a_1,a_2,a_{\rm{c}},r$) and under the constant volume constraints $V_1 = \bar{V} - \delta V, V_2 = \bar{V} + \delta V$ in Mathematica~\cite{Mathematica}(\textcolor{red}{link}). We computed the contact area $A_{\rm{c}}=4\pi H_c$ for values of $\gamma_{\rm{c}}/2\bar{\gamma}_{\rm{f}}$ evenly spaced on the interval $[0,1]$. From these results, we fit the contact area as a function of the tension ratio [Fig.~\ref{fig:asymmetry_doublet_parameterization}(c)], because our implementation of the numerical continuation method to obtain bifurcation lines requires an explicit expression that relates the contact area to the interfacial tensions. For unequal volumes ($V_1 \neq V_2$), but identical outer surface tensions, we used a 5th order polynomial to fit a function $A_{\rm{c}} = A_{\rm{c}}(\gamma_{\rm{c}}/2\bar{\gamma}_{\rm{f}})$ on the interval $[0,1]$ using Mathematica's function \emph{Fit} with the default \emph{LevenbergMarquardt} method [Fig.~\eqref{fig:asymmetry_doublet_parameterization}(c)].
For droplets with asymmetric outer tension, but equal volumes, the droplet with higher outer tension is completely internalized if $\gamma_{\rm{c}}/2\bar{\gamma}_{\rm{f}} \leq \delta \gamma_{\rm{f}}$ \cite{maitre2016asymmetric}, thus, we used a piecewise function to fit the contact area with $A_{\rm{c}} = 2^{4/3} A_0$ on the interval $[0,\delta \gamma_{\rm{f}}]$. The interval $[\delta \gamma_{\rm{f}},1]$ was fitted with a combination of a rational function of the form $a + b/(\gamma_{\rm{c}}/2\gamma_{\rm{f}} - c)^d$ close to the threshold of internalization with fit parameters $a-d$ and a 5th order polynomial [Fig.~\ref{fig:asymmetry_doublet_parameterization}(c)]. Fits of the contact area were then used for continuation in MatCont and simulations in Mathematica to derive the state diagrams shown in Fig.~\ref{fig:6}. 

All codes are available at \textcolor{red}{link}.

\section{Literature values for reaction and diffusion rates}

Khait et al. 2016 obtained quantitative estimates for many parameters governing the dynamics of Notch receptors and ligands (Tab.~\ref{tab:parameter_values}, \cite{khait2016quantitative}). The authors measured the 2D diffusion constant $D_{\mathrm{m}}$ and the endocytosis rate $k_{\rm{off}}$ in different cell lines and estimated the reaction rates from previously reported measurements of the binding kinetics for soluble molecules in 3D. The rate of receptor and ligand transport from the bulk to the surface $k_{\rm{on}}^{\rm{R}} c_{\rm{R}}^0$ and $k_{\rm{on}}^{\rm{L}} c_{\rm{L}}^0$ were estimated by assuming that the steady-state surface densities are $m_{\rm{R}}^0=\SI{100}{\per\micro\metre\squared}$ and $m_{\rm{L}}^0=\SI{10}{\per\micro\metre\squared}$ (i.e. there is an excess of receptors) when a cell is not in contact with another cell or ligand-coated substrate. In that case $m_{\rm{R}}=m_{\rm{R}}^0=k_{\rm{on}}^{\rm{R}} c_{\rm{R}}^0/k_{\rm{off}}^{\rm{R}}$ and $m_{\rm{L}}=m_{\rm{L}}^0=k_{\rm{on}}^{\rm{L}} c_{\rm{L}}^0/k_{\rm{off}}^{\rm{L}}$.
%Parameter $b$ gives the typical radius of a cellular contact as reported in \cite{khait2016quantitative}.
$A_{\rm{c}}$ gives the range of contact areas for two spherical cells with radius $\SI{5}{\micro\metre}$ that keep a normalized contact area $A_{\rm{c}}/A_0 \in [0,1]$ as assumed in this work.

\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
        Parameter&  Symbol& Value \\
        \hline 
        Endocytosis&  $k_{\rm{off}}$ & \SI{0.02}{\per\second}\\
        Cleavage &  $k_{\rm{s}}$ & \SI{0.34}{\per\second} \\
        Binding &  $k_+$ & \SI{0.167}{\micro\metre\squared\per\second}\\
        Unbinding &  $k_-$& \SI{0.034}{\per\second}\\
        Diffusion coefficients &   $D_{m_{\rm{R}}},  D_{m_{\rm{L}}}$ & \SIrange{0.02}{0.08}{\micro\metre\squared\per\second}\\
        Diffusion coefficient &  $D_{m_\mathrm{RL}}$ & $(D_{m_\mathrm{R}} + D_{m_\mathrm{L}})/4$\\
        Exocytosis receptors &  $k_{\rm{on}}^{\rm{R}} c_{\rm{R}}^0$ & \SI{2}{\per\micro\metre\squared\per\second}\\
        Exocytosis ligands &  $k_{\rm{on}}^{\rm{L}} c_{\rm{L}}^0$ & \SI{0.2}{\per\micro\metre\squared\per\second}\\
        %Contact radius &  $b$ & \SIrange{0.01}{3}{\micro\metre}\\
        Contact area &  $A_{\rm{c}}$ & \SIrange{0}{125}{\micro\metre\squared}\\
        \hline
    \end{tabular}
    \caption{Typical parameter values for reaction and diffusion rates of receptor and ligand molecules as reported in \cite{khait2016quantitative} and estimate of common cellular length scales}
    \label{tab:parameter_values}
\end{table}

\begin{figure}
    \centering
    \includegraphics{Figures/SymmetryBreaking.png}
    \caption{(a) Uniform fixpoints of Eq.~\eqref{eq:u_ode} computed numerically (gray) and approximation from linearization of the response function $\sigma(s_{ij})$ around $s_{ij}=1$ [Eq.~\eqref{eq:uniform_steady_states}], (orange), $h=4$. (b) Comparison between Eq.~\eqref{eq:symmetry_breaking_scaling} (orange) and the steady-state contact area computed numerically along the supercritical pitchfork bifurcation line derived via continuation in MatCont (gray)}
    \label{fig:symmetry_breaking}
\end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[]{Figures/SteadyStateContactArea.png}
    \caption{State diagram as shown in Fig.~\ref{fig:5}(a) for $\gamma_0/2\gamma_{\rm{f}} = 0.98$. The color code indicates the normalized contact area at the fixpoint, i.e. at the uniform fixpoint state below the PF and SHET line and at the symmetry-broken fixpoints above the PF and Hopf line. The oscillatory regime between Hopf and SHET line is white as it does not contain any stable fixpoints.}
    \label{fig:SteadyStateContactArea}
\end{figure}

\section{Experimental methods (Fig.~\ref{fig:1}(a))}
\label{sec:experimental_methods}

\subsection{Cell culturing}
NIH/3T3 fibroblasts (ATCC CRL-1658, strain: NIH/Swiss) were cultured in \SI{10}{\centi\metre} plastic petri dishes at 37$^{\circ}$C and 5\% CO2 in phenol-red free DMEM medium containing 10\%FCS (in the following just called ”medium”). Cells were passaged every 2-3 days at $\sim~80-90\%$ confluency by washing with dPBS followed by \SIrange{2}{3}{\minute} incubation with \SI{1}{\milli\litre} Trypsin at 37$^{\circ}$C. Detached cells were resuspended in \SIrange{4}{5}{\milli\litre} medium and added either to a new \SI{10}{\centi\metre} petri dish with \SI{10}{\milli\litre} medium for culturing or a 6-well plate with \SI{2}{\milli\litre} medium per well for experiments, yielding a final confluency of 10-20\%.

\subsection{Imaging cells on micropatterns (Fig.~\ref{fig:1}(a))}
3T3 fibroblasts were seeded on Fibronectin-coated micropatterns of \SI{10}{\micro\metre} diameter as described in \cite{lembo2023distance}. Seeded cells were washed with dPBS and then phenol-red free DMEM medium with \SI{10}{\micro\gram\per\milli\litre} Hoechst33342 (1:1000 from \SI{10}{\milli\gram\per\milli\litre} in DMSO) and \SI{1}{\micro\mole} SiR-actin added to the dish. Cells were imaged $\geq\SI{30}{\minute}$ after adding the live dyes using a SP5 Confocal Microscope (Leica) with a 100x oil-immersion objective (1.4 NA).

